Properties of optically selected BL Lac candidates from the SDSS

\textbf{Context.} Deep optical surveys open the avenue for find large numbers of BL Lac objects that are hard to identify because they lack the unique properties classifying them as such. While radio or X-ray surveys typically reveal dozens of sources, recent compilations based on optical criteria alone have increased the number of BL Lac candidates considerably. However, these compilations are subject to biases and may contain a substantial number of contaminating sources. \textbf{Aims.} In this paper we extend our analysis of 182 optically selected BL Lac object candidates from the SDSS with respect to an earlier study. The main goal is to determine the number of bona fide BL Lac objects in this sample. \textbf{Methods.} We examine their variability characteristics, determine their broad-band radio-UV SEDs, and search for the presence of a host galaxy. In addition we present new optical spectra for 27 targets with improved S/N with respect to the SDSS spectra. \textbf{Results.} At least 59% of our targets have shown variability between SDSS DR2 and our observations by more than 0.1-0.27 mag de- pending on the telescope used. A host galaxy was detected in 36% of our targets. The host galaxy type and luminosities are consistent with earlier studies of BL Lac host galaxies. Simple fits to broad-band SEDS for 104 targets of our sample derived synchrotron peak frequencies between $13.5 \leq \mathrm{log}_{10}(\nu_{\mathrm{peak}}) \leq 16$ with a peak at $\mathrm{log}_{10} \sim 14.5$. Our new optical spectra do not reveal any new redshift for any of our objects. Thus the sample contains a large number of bona fide BL Lac objects and seems to contain a substantial fraction of intermediate-frequency peaked BL Lacs.

==> finalTable_orig.tex <==
%\begin{longtable}{c|c|c|c|c|c|c|c|c|c|c|c|c}
\begin{longtable}{ccccccccccccc}
%\centering
%\caption{}
%\begin{tabular}
\caption {Total summary of available properties of all objects. This table will be also published in electronical form. Despite the target name, the
SDSS redshift with its respective uncertainty flag, the X-ray and radio indices from RASS and FIRST/NVSS are shown. All those properties are
obtained from the paper of C05. Adjacently the corrected polarization from paper I (with its respective error) as well as the variation limit (VL)
and the variation are given. Also the core fraction with its respective error (flag ``u'' is for undetected) and the peak frequencies obtained by the
SED fits as well as their respective flags are given. The flags indicate whether the peak estimate is uncertain due to the shallowness of the radio
data (``radio'' if only one or no radio point available), or due to the presence of a strong host galaxy if the host galaxy fraction exceeds 0.5 (flag is
``galaxy'').\label{summaryAllProps}}\\
%\toprule
Target name & z$_{\text{SDSS}}$ & z$_{\text{SDSS}}$ & aox & aro & pol & ePol & VL & Var & core & error & log$\left(\nu_\text{Peak}\right)$ & SED \tabularnewline 
 & & Flag & & &  & &  &  & frac & frac & & Flag \tabularnewline
%\hline
$[$SDSS J$]$ &  &  &  &  & $[$\%$]$ & $[$\%$]$ & $[$mag$]$ & $[$mag$]$ &  &  & $[$log$\left(\text{Hz}\right)]$ & \tabularnewline
\hline
\hline
\endfirsthead
\caption* {\textbf{Table \ref{summaryAllProps}} $-$ Continued.}\\
%\toprule
Target name & z$_{\text{SDSS}}$ & z$_{\text{SDSS}}$ & aox & aro & pol & ePol & VL & Var & core & error & log$\left(\nu_\text{Peak}\right)$ & SED \tabularnewline 
 & & Flag & & &  & &  &  & frac & frac & & Flag \tabularnewline
%\hline
$[$SDSS J$]$ &  &  &  &  & $[$\%$]$ & $[$\%$]$ & $[$mag$]$ & $[$mag$]$ &  &  & $[$log$\left(\text{Hz}\right)]$ & \tabularnewline
\hline
\hline
\endhead
\endfoot
%\bottomrule
\endlastfoot
000121.47$-$001140.3 & 0.4620 & - & $>$0.98 & 0.63 & 4.34 & 0.75 & 0.06 & -0.103 & 0.60 & 0.07 & 16.59 & - \tabularnewline
002142.26$-$090044.4 & 0.6481 & - & $>$1.07 & 0.51 & 12.80 & 0.83 & 0.065 & 0.104 & 1 & u & - & - \tabularnewline 
002200.95+000658.0 & 0.3057 & - & 0.94 & 0.28 & $<$2.56 & - & 0.064 & 0.259 & $<$0.16 & 0.07 & 15.21 & radio \tabularnewline 
002839.77+003542.2 & 0.6866 & u & $>$1.00 & 0.49 & 4.45 & 0.69 & 0.072 & 0.519 & 0.85 & 0.10 & 17.43 & - \tabularnewline 
003514.72+151504.1 & - & - & 1.16 & 0.25 & 6.90 & 0.96 & 0.087 & 1.057 & 1 & u & 17.29 & radio \tabularnewline 
004054.65$-$091526.8 & 5.0300 & - & $>$1.01 & $<$0.05 & $<$3.99 & - & 0.126 & 0.105 & 1 & u & - & - \tabularnewline 
005041.31$-$092905.1 & - & - & 1.28 & 0.55 & 19.01 & 0.35 & 0.05 & -0.641 & 1 & u & 15.08 & radio \tabularnewline 
010058.19$-$005547.8 & $>$0.6679 & u & $>$1.04 & 0.49 & 12.82 & 0.66 & 0.057 & -0.262 & 1 & u & 13.53 & - \tabularnewline 
010326.01+152624.8 & 0.2461 & - & $>$1.22 & 0.60 & 1.62 & 0.68 & 0.068 & 0.669 & 0.25 & 0.04 & 16.81 & radio \tabularnewline 
011012.66$-$004746.9 & 0.5477 & - & $>$0.94 & 0.54 & 5.52 & 0.90 & 0.074 & 0.122 & 0.69 & 0.05 & 14.34 & - \tabularnewline 
011452.77+132537.5 & - & - & $>$1.34 & 0.41 & 9.10 & 0.61 & 0.057 & 0.801 & 1 & u & 14.8 & radio \tabularnewline 
012155.87$-$102037.2 & 0.4695 & - & $>$1.02 & $<$0.23 & $<$0.90 & - & 0.06 & 0.005 & $<$0.20 & 0.08 & - & - \tabularnewline 
012227.38+151023.1 & - & - & $>$0.89 & 0.55 & 10.41 & 1.05 & 0.07 & 0.557 & 1 & u & 13.63 & - \tabularnewline 
012716.31$-$082128.9 & 0.3620 & u & $>$1.04 & 0.66 & 6.32 & 0.87 & 0.067 & 0.203 & 1 & u & - & - \tabularnewline 
012750.83$-$001346.6 & 0.4376 & - & $>$0.98 & 0.40 & 4.13 & 0.78 & 0.07 & -0.032 & 0.39 & 0.09 & 14.33 & radio \tabularnewline 
013408.95+003102.5 & - & - & $>$0.93 & $<$0.29 & $<$2.03 & - & 0.067 & 0.035 & 1 & u & - & - \tabularnewline 
014125.83$-$092843.7 & $>$0.5000 & u & 1.45 & 0.60 & 4.88 & 0.56 & 0.067 & 0.88 & 1 & u & 13.93 & - \tabularnewline 
020106.18+003400.2 & 0.2985 & - & 0.89 & 0.38 & 1.37 & 0.67 & 0.061 & 0.424 & 0.49 & 0.09 & 15.83 & radio \tabularnewline 
020137.66+002535.1 & - & - & $>$0.99 & $<$0.26 & $<$2.18 & - & 0.065 & 0.109 & 1 & u & - & - \tabularnewline 
022048.46$-$084250.4 & 0.5252 & u & 1.09 & 0.49 & 6.09 & 0.45 & 0.054 & -0.355 & 1 & u & 19.42 & - \tabularnewline 
023813.68$-$092431.4 & 0.4188 & - & 1.09 & 0.34 & 2.51 & 0.70 & 0.067 & 0.205 & $<$0.07 & 0.06 & 14.52 & galaxy \tabularnewline 
024156.38+004351.6 & 0.9900 & - & $>$0.90 & 0.11 & 2.60 & 0.72 & 0.06 & 0.026 & 1 & u & - & - \tabularnewline 
024157.37+000944.1 & 0.7896 & u & 0.83 & 0.32 & 4.03 & 1.63 & 0.114 & 0.303 & 1 & u & 14.14 & radio \tabularnewline 
024302.93+004627.3 & 0.4089 & - & $>$0.96 & 0.53 & $<$3.17 & - & 0.07 & 0.106 & 0.33 & 0.09 & - & - \tabularnewline 
024752.13+004106.3 & 0.3929 & - & $>$0.82 & 0.41 & $<$2.40 & - & 0.066 & -0.086 & 0.44 & 0.07 & 13.91 & radio \tabularnewline 
025046.48$-$005449.0 & - & - & $>$0.74 & $<$0.28 & $<$2.95 & - & 0.082 & 0.095 & 1 & u & - & - \tabularnewline 
025612.47$-$001057.8 & 0.6302 & - & $>$-0.11 & $<$0.28 & $<$2.42 & - & 0.076 & -0.284 & 0.62 & 0.07 & 14.11 & radio \tabularnewline 
030235.78$-$075027.0 & - & - & $>$0.71 & 0.45 & 8.42 & 0.71 & 0.064 & -0.497 & 1 & u & - & - \tabularnewline 
030240.30+003849.9 & - & - & $>$0.73 & 0.33 & $<$1.93 & - & 0.066 & 0.041 & 1 & u & 14.04 & - \tabularnewline 
030433.96$-$005404.7 & 0.5112 & - & 1.03 & 0.44 & 1.83 & 0.60 & 0.059 & -0.211 & 0.80 & 0.14 & 14.99 & radio \tabularnewline 
031712.23$-$075850.4 & 2.6993 & - & $>$1.03 & - & $<$3.20 & - & 0.076 & 0.075 & 1 & u & - & - \tabularnewline 
032343.62$-$011146.1 & - & - & 1.35 & 0.32 & 5.22 & 0.98 & 0.067 & 0.789 & 1 & u & 15.4 & radio \tabularnewline 
032356.64$-$010829.6 & 0.3923 & - & 0.89 & 0.41 & $<$2.13 & - & 0.071 & 0.052 & 0.50 & 0.07 & 13.38 & radio \tabularnewline 
040911.36$-$055529.4 & - & - & $>$0.93 & 0.53 & 9.76 & 1.33 & 0.079 & 0.629 & 1 & u & - & - \tabularnewline 
045128.96$-$002911.5 & - & - & $>$0.75 & 0.80 & $<$3.98 & - & 0.078 & 0.138 & 1 & u & - & - \tabularnewline 
074054.60+322601.0 & $>$0.9460 & u & $>$1.09 & 0.38 & 5.44 & 0.83 & 0.051 & 0.002 & 1 & u & - & - \tabularnewline 
075144.94+392817.6 & 0.4338 & u & $>$0.80 & 0.44 & 3.99 & 1.78 & 0.099 & -0.921 & 1 & u & - & - \tabularnewline 
075602.72+414039.8 & 0.5788 & - & $>$0.94 & 0.36 & $<$6.09 & - & 0.106 & -0.216 & 1 & u & - & - \tabularnewline 
081840.06+315348.2 & - & - & $>$1.01 & 0.57 & 14.48 & 1.17 & 0.077 & -0.381 & 1 & u & - & - \tabularnewline 
083413.90+511214.7 & - & - & $>$1.05 & 0.26 & $<$5.61 & - & 0.092 & -0.156 & 1 & u & - & - \tabularnewline 
083918.75+361856.1 & 0.3343 & - & $>$0.95 & 0.40 & $<$2.92 & - & 0.061 & 0.066 & 0.42 & 0.09 & 18.42 & galaxy \tabularnewline 
084225.52+025252.7 & 0.4251 & - & 1.15 & 0.45 & $<$1.57 & - & 0.033 & 0.155 & 0.45 & 0.04 & 17.53 & radio \tabularnewline 
084908.81+020622.5 & - & - & $>$1.06 & 0.55 & 10.94 & 0.71 & 0.033 & 0.206 & 1 & u & 13.79 & radio \tabularnewline 
085638.50+014000.7 & 0.4479 & - & $>$1.03 & 0.38 & $<$3.78 & - & 0.034 & 0.088 & 0.66 & 0.07 & 13.33 & - \tabularnewline 
085749.80+013530.3 & 0.2812 & - & 1.20 & 0.51 & 4.50 & 0.68 & 0.031 & 0.051 & 0.39 & 0.05 & 14.97 & radio \tabularnewline 
085920.56+004712.1 & - & - & 0.84 & 0.52 & 4.20 & 0.91 & 0.057 & 0.518 & 1 & u & 14.98 & radio \tabularnewline 
090133.43+031412.5 & 0.4591 & - & $>$1.04 & $<$0.21 & $<$2.08 & - & 0.033 & 0.03 & 1 & u & 20.39 & radio \tabularnewline 
090939.84+020005.3 & - & - & $>$1.00 & 0.73 & 18.99 & 0.49 & 0.035 & -1.101 & 1 & u & 13.33 & radio \tabularnewline 
091848.57+021321.8 & - & - & $>$1.13 & 0.32 & 4.29 & 1.16 & 0.058 & 0.896 & 1 & u & 14.49 & radio \tabularnewline 
092542.87+595816.3 & - & - & 1.03 & 0.40 & 8.65 & 1.10 & 0.078 & 0.171 & 1 & u & - & - \tabularnewline 
092638.88+541126.7 & 0.8500 & u & $>$1.09 & 0.51 & 7.02 & 0.93 & 0.077 & -0.55 & 1 & u & - & - \tabularnewline 
092912.25+030029.9 & - & - & $>$1.00 & 0.24 & 9.41 & 0.69 & 0.04 & -0.345 & 1 & u & 12.9 & radio \tabularnewline 
094245.30+541620.4 & - & - & $>$0.99 & 0.45 & 7.51 & 2.17 & 0.104 & 0.024 & 1 & u & 15.39 & - \tabularnewline 
094257.81$-$004705.2 & 1.3600 & - & $>$1.02 & 0.23 & $<$1.62 & - & 0.033 & -0.229 & 1 & u & 13.84 & radio \tabularnewline 
094432.33+573536.2 & - & - & 0.85 & 0.32 & 3.41 & 1.29 & 0.088 & -0.32 & 0.73 & 0.10 & - & - \tabularnewline 
094432.33+573536.2 & - & - & 0.85 & 0.32 & 8.06 & 0.61 & 0.088 & -0.32 & 0.73 & 0.10 & - & - \tabularnewline 
094441.48+555753.1 & - & - & $>$1.05 & 0.53 & $<$4.48 & - & 0.088 & -0.198 & 1 & u & - & - \tabularnewline 
094542.24+575747.7 & 0.2289 & - & 1.53 & 0.48 & 4.90 & 0.22 & 0.04 & -0.532 & 0.72 & 0.11 & 14.87 & - \tabularnewline 
094620.21+010452.1 & 0.5775 & - & 0.81 & 0.42 & 4.86 & 0.56 & 0.038 & -0.516 & 0.74 & 0.13 & 14.03 & radio \tabularnewline 
095127.82+010210.2 & - & - & 1.13 & 0.46 & 4.36 & 0.69 & 0.057 & -0.029 & 0.55 & 0.12 & 15.58 & - \tabularnewline 
095649.53+015601.8 & - & - & 0.80 & 0.43 & 7.10 & 1.60 & 0.043 & 0.403 & 1 & u & 16.01 & - \tabularnewline 
100050.22+574609.1 & 0.6392 & - & $>$1.16 & 0.58 & 5.14 & 1.22 & 0.088 & 0.311 & 1 & u & 13.63 & - \tabularnewline 
100326.63+020455.7 & - & - & $>$1.00 & 0.38 & 10.21 & 1.07 & 0.035 & 0.363 & 1 & u & 14.62 & - \tabularnewline 
100612.23+644011.6 & - & - & 1.07 & 0.53 & 8.81 & 1.01 & 0.074 & -0.49 & 1 & u & - & - \tabularnewline 
100959.63+014533.8 & $>$1.0900 & u & $>$0.99 & 0.55 & 14.98 & 1.35 & 0.038 & 1.034 & 1 & u & 13.36 & - \tabularnewline 
101115.64+010642.7 & 0.8615 & u & $>$0.95 & 0.70 & $<$1.64 & - & 0.058 & 0.203 & 1 & u & 14.31 & radio \tabularnewline 
101858.55+591127.8 & - & - & $>$1.40 & 0.50 & 19.08 & 0.46 & 0.046 & 0.102 & 1 & u & 19.47 & - \tabularnewline 
101950.87+632001.6 & - & - & $>$1.28 & 0.56 & 7.80 & 0.65 & 0.072 & -0.885 & 1 & u & 13.68 & - \tabularnewline 
102013.78+625010.1 & 0.2495 & - & 1.22 & 0.49 & $<$3.77 & - & 0.076 & 0.236 & 0.35 & 0.05 & - & - \tabularnewline 
102243.73$-$011302.5 & - & - & 0.93 & 0.39 & $<$2.56 & - & 0.031 & -0.122 & 1 & u & 20.08 & radio \tabularnewline 
102523.04+040229.0 & 0.2078 & - & 1.11 & 0.52 & 1.49 & 0.61 & 0.032 & 0.171 & 0.44 & 0.04 & 15.36 & radio \tabularnewline 
102724.97+631753.1 & $>$0.5816 & - & 1.14 & 0.41 & 11.51 & 1.06 & 0.077 & -0.181 & 1 & u & - & - \tabularnewline 
103208.36+040157.0 & - & - & $>$0.99 & 0.65 & 11.84 & 0.49 & 0.057 & -0.024 & 1 & u & - & - \tabularnewline 
103220.29+030949.2 & 0.3233 & - & $>$1.18 & 0.45 & 4.92 & 0.71 & 0.032 & 0.371 & 0.81 & 0.09 & 13.8 & radio \tabularnewline 
103239.07+662323.3 & - & - & $>$1.13 & 0.60 & 3.26 & 1.09 & 0.074 & -0.074 & 1 & u & - & - \tabularnewline 
103940.70+053609.3 & 0.5103 & - & $>$0.73 & 0.38 & $<$4.01 & - & 0.032 & -1.026 & 0.52 & 0.10 & 15.01 & radio \tabularnewline 
104523.86+015722.1 & - & - & $>$0.96 & 0.30 & $<$1.61 & - & 0.033 & -0.186 & 1 & u & - & - \tabularnewline 
104833.57+620305.0 & - & - & $>$1.07 & $<$0.27 & $<$1.72 & - & 0.055 & -0.296 & 1 & u & - & - \tabularnewline 
105151.84+010310.7 & 0.2654 & - & $>$1.06 & 0.42 & 1.92 & 0.35 & 0.034 & -0.74 & 0.84 & 0.07 & 14.21 & radio \tabularnewline 
105151.84+010310.7 & 0.2654 & - & $>$1.06 & 0.42 & 4.86 & 0.33 & 0.034 & -0.74 & 0.84 & 0.07 & 14.21 & radio \tabularnewline 
105606.62+025213.5 & 0.2360 & - & 0.72 & 0.32 & 1.16 & 0.39 & 0.056 & 0.089 & 0.36 & 0.06 & 15.77 & - \tabularnewline 
105752.79$-$005908.3 & 0.4678 & u & 0.94 & 0.29 & $<$3.90 & - & 0.033 & 0.254 & 0.72 & 0.13 & 15.37 & radio \tabularnewline 
105829.62+013358.8 & 0.8862 & u & 1.16 & 0.76 & 15.10 & 0.27 & 0.031 & -1.712 & 1 & u & 12.77 & radio \tabularnewline 
110356.15+002236.4 & 0.2747 & - & $>$1.12 & 0.52 & 4.38 & 0.36 & 0.056 & 0.192 & 0.40 & 0.03 & 14.89 & galaxy \tabularnewline 
110704.78+501037.9 & 0.7061 & - & $>$1.14 & 0.49 & 4.27 & 1.66 & 0.095 & 0.035 & 0.48 & 0.11 & - & - \tabularnewline 
110735.92+022224.5 & $>$1.0750 & u & $>$1.09 & 0.40 & 9.39 & 0.42 & 0.032 & -0.233 & 1 & u & 14.59 & radio \tabularnewline 
111717.55+000633.6 & 0.4511 & - & 0.87 & 0.44 & 1.46 & 0.52 & 0.036 & 0.803 & 0.67 & 0.08 & 15.46 & radio \tabularnewline 
111717.55+000633.6 & 0.4511 & - & 0.87 & 0.44 & 1.87 & 0.52 & 0.036 & 0.803 & 0.67 & 0.08 & 15.46 & radio \tabularnewline 
113115.50+023450.2 & $>$0.4538 & u & $>$1.16 & 0.38 & $<$2.79 & - & 0.033 & 0.811 & 1 & u & 14.22 & - \tabularnewline 
113234.38+023740.3 & - & - & $>$1.02 & 0.59 & $<$1.83 & - & 0.034 & 0.078 & 1 & u & 17.99 & radio \tabularnewline 
113245.61+003427.7 & - & - & 1.48 & 0.61 & 6.35 & 0.68 & 0.056 & 0.092 & 1 & u & 13.54 & radio \tabularnewline 
113523.70+660941.0 & - & - & $>$1.18 & 0.56 & 13.52 & 2.16 & 0.051 & 0.731 & 1 & u & - & - \tabularnewline 
113523.70+660941.0 & - & - & $>$1.18 & 0.56 & 12.43 & 0.83 & 0.051 & 0.731 & 1 & u & - & - \tabularnewline 
114153.35+021924.4 & 3.5979 & - & $>$1.19 & 0.11 & $<$1.26 & - & 0.056 & 0.223 & 1 & u & 13.91 & radio \tabularnewline 
114312.11+612210.8 & - & - & 1.46 & 0.48 & 5.97 & 0.97 & 0.072 & -0.701 & 1 & u & 13.63 & - \tabularnewline 
114926.13+624332.5 & 0.7620 & u & $>$1.16 & 0.41 & 4.88 & 1.81 & 0.046 & 0.656 & 1 & u & - & - \tabularnewline 
114926.13+624332.5 & 0.7620 & u & $>$1.16 & 0.41 & 7.94 & 0.60 & 0.046 & 0.656 & 1 & u & - & - \tabularnewline 
115404.54$-$001009.9 & 0.2535 & - & 0.95 & 0.37 & 2.19 & 0.69 & 0.031 & -0.086 & 0.55 & 0.07 & 14.6 & - \tabularnewline 
115548.41+613554.0 & - & - & $>$1.15 & 0.30 & $<$8.91 & - & 0.124 & 0.612 & 1 & u & - & - \tabularnewline 
115548.41+613554.0 & - & - & $>$1.15 & 0.30 & 3.73 & 1.18 & 0.124 & 0.612 & 1 & u & - & - \tabularnewline 
120303.50+603119.1 & 0.0653 & - & 1.44 & 0.49 & $<$1.57 & - & 0.073 & 0.627 & 0.46 & 0.03 & 14.62 & galaxy \tabularnewline 
120658.03+052952.2 & $>$0.7911 & - & $>$1.08 & 0.75 & 7.47 & 1.07 & 0.038 & 0.682 & 1 & u & 14.41 & radio \tabularnewline 
120938.33+021017.2 & - & - & 1.02 & 0.39 & 3.21 & 1.24 & 0.059 & 0.642 & 1 & u & 16.67 & radio \tabularnewline 
121221.56+534128.0 & 3.1900 & - & $>$1.22 & $<$0.03 & $<$0.69 & - & 0.042 & 0.154 & 1 & u & - & - \tabularnewline 
121300.80+512935.6 & 0.7957 & u & 1.08 & 0.45 & 13.38 & 1.17 & 0.075 & 0.16 & 1 & u & 14.57 & radio \tabularnewline 
121348.81+642520.2 & $>$0.4157 & - & $>$1.07 & 0.43 & 22.01 & 1.83 & 0.133 & 0.419 & 1 & u & - & - \tabularnewline 
121500.80+500215.6 & - & - & $>$1.38 & 0.44 & 8.00 & 1.57 & 0.04 & 0.254 & 1 & u & - & - \tabularnewline 
121500.80+500215.6 & - & - & $>$1.38 & 0.44 & 13.55 & 0.22 & 0.04 & 0.254 & 1 & u & - & - \tabularnewline 
121649.97+054136.7 & - & - & $>$1.03 & 0.59 & 16.66 & 0.88 & 0.035 & 0.135 & 1 & u & 13.96 & radio \tabularnewline 
121758.72$-$002946.2 & 0.4188 & - & $>$1.16 & 0.62 & 11.88 & 0.97 & 0.034 & 1.034 & 0.59 & 0.08 & 13.19 & radio \tabularnewline 
121834.93$-$011954.3 & 0.5545 & u & $>$0.95 & 0.56 & 11.24 & 0.36 & 0.055 & -0.607 & 1 & u & 13.75 & radio \tabularnewline 
121944.98+044622.4 & 0.4891 & - & $>$1.31 & 0.33 & 5.22 & 0.63 & 0.031 & 0.441 & 0.84 & 0.08 & 14.39 & - \tabularnewline 
121945.70$-$031424.0 & 0.2987 & - & 1.08 & 0.37 & 7.10 & 0.31 & 0.031 & -0.936 & 1 & u & 14.3 & - \tabularnewline 
122012.14$-$000306.8 & - & - & 1.07 & 0.42 & 6.65 & 0.82 & 0.034 & 0.369 & 1 & u & 16.74 & radio \tabularnewline 
122300.31+515313.9 & 0.3650 & - & $>$1.06 & 0.36 & 4.02 & 1.16 & 0.081 & 0.018 & 0.57 & 0.05 & - & - \tabularnewline 
122809.13$-$022136.1 & 0.3227 & - & 0.96 & 0.27 & $<$1.63 & - & 0.033 & 0.088 & 0.27 & 0.06 & 15.47 & radio \tabularnewline 
123132.38+013814.0 & 3.2300 & - & $>$1.17 & 0.23 & 1.48 & 0.67 & 0.059 & 0.173 & 1 & u & 20.99 & radio \tabularnewline 
123132.38+013814.0 & 3.2300 & - & $>$1.17 & 0.23 & $<$2.93 & - & 0.059 & 0.173 & 1 & u & 20.99 & radio \tabularnewline 
123341.33$-$014423.7 & - & - & $>$1.17 & 0.45 & 10.64 & 0.64 & 0.032 & 0.406 & 1 & u & 14.35 & radio \tabularnewline 
123743.09+630144.9 & 3.5347 & - & $>$1.18 & $<$0.04 & $<$1.38 & - & 0.046 & 0.146 & 1 & u & - & - \tabularnewline 
124225.39+642919.1 & 0.0424 & - & $>$1.40 & - & $<$1.49 & - & 0.074 & 0.342 & $<$0.05 & 0.05 & - & - \tabularnewline 
124425.30+044459.7 & 0.3999 & - & $>$1.01 & 0.41 & 2.33 & 0.78 & 0.035 & 0.213 & $<$0.16 & 0.07 & 13.57 & galaxy \tabularnewline 
124533.79+022825.2 & $>$1.0900 & u & $>$1.04 & 0.45 & 5.95 & 0.50 & 0.033 & -0.14 & 1 & u & - & - \tabularnewline 
124602.52+011318.8 & 0.3864 & - & $>$1.36 & 0.42 & 3.37 & 0.78 & 0.059 & 1.838 & 1 & u & 14.06 & radio \tabularnewline 
124834.30+512807.8 & 0.3508 & - & 1.41 & 0.50 & 8.13 & 1.36 & 0.078 & 0.188 & 0.71 & 0.11 & 14.0 & - \tabularnewline 
125032.59+021632.2 & - & - & $>$0.97 & 0.75 & 9.70 & 0.98 & 0.035 & 0.929 & 1 & u & 13.65 & radio \tabularnewline 
125359.32+624257.5 & $>$0.8680 & - & 1.25 & 0.37 & 17.28 & 1.18 & 0.089 & -0.215 & 1 & u & - & - \tabularnewline 
125820.79+612045.6 & 0.2235 & - & $>$1.19 & 0.39 & $<$1.62 & - & 0.08 & -0.346 & $<$0.00 & 0.00 & - & - \tabularnewline 
131106.48+003510.0 & - & - & 1.19 & 0.38 & 13.80 & 0.53 & 0.031 & 0.095 & 1 & u & 14.86 & radio \tabularnewline 
131330.15+020105.9 & 0.3558 & - & 1.22 & 0.52 & 5.58 & 0.53 & 0.032 & 0.042 & 0.73 & 0.04 & 14.67 & radio \tabularnewline 
132301.01+043951.4 & 0.2244 & - & 0.96 & 0.45 & 1.39 & 0.53 & 0.031 & -0.093 & 0.58 & 0.05 & 14.09 & radio \tabularnewline 
132541.91$-$022810.1 & 0.8073 & u & 0.82 & 0.43 & 5.21 & 1.04 & 0.067 & 0.318 & 1 & u & 14.08 & radio \tabularnewline 
132759.76+645811.3 & 0.4468 & - & $>$1.11 & 0.52 & $<$2.99 & - & 0.092 & -0.069 & $<$0.04 & 0.06 & - & - \tabularnewline 
133105.71$-$002221.2 & 0.2426 & - & 1.23 & 0.40 & 1.83 & 0.55 & 0.032 & 0.04 & 0.14 & 0.04 & 14.52 & radio \tabularnewline 
133219.65+622715.9 & 3.1500 & - & $>$1.10 & 0.19 & $<$1.68 & - & 0.089 & -0.045 & 1 & u & - & - \tabularnewline 
134037.59$-$014847.6 & 0.5130 & - & $>$0.98 & 0.43 & 4.10 & 0.70 & 0.038 & -0.355 & 0.69 & 0.09 & 14.08 & radio \tabularnewline 
135738.70+012813.6 & 0.5640 & u & 1.11 & 0.46 & 9.08 & 0.33 & 0.041 & 0.552 & 1 & u & 15.26 & radio \tabularnewline 
135738.70+012813.6 & 0.5640 & u & 1.11 & 0.46 & 9.18 & 3.01 & 0.041 & 0.552 & 1 & u & 15.26 & radio \tabularnewline 
140450.91+040202.2 & - & - & 1.26 & 0.32 & 7.75 & 0.77 & 0.032 & 0.744 & 1 & u & - & - \tabularnewline 
141003.92+051557.7 & 0.5440 & - & $>$0.49 & 0.40 & 1.31 & 0.59 & 0.035 & -0.044 & 0.55 & 0.04 & 14.3 & radio \tabularnewline 
141004.65+020306.9 & $>$1.1150 & u & $>$1.26 & 0.56 & 3.16 & 0.90 & 0.055 & 1.491 & 1 & u & 13.11 & radio \tabularnewline 
141004.65+020306.9 & $>$1.1150 & u & $>$1.26 & 0.56 & $<$6.76 & - & 0.055 & 1.491 & 1 & u & 13.11 & radio \tabularnewline 
141030.84+610012.8 & 0.3833 & - & 0.89 & 0.36 & $<$3.10 & - & 0.08 & 0.175 & 0.36 & 0.06 & 15.67 & radio \tabularnewline 
141826.33$-$023334.1 & - & - & $>$1.41 & 0.34 & 2.84 & 0.44 & 0.031 & 0.233 & 1 & u & 14.18 & - \tabularnewline 
141927.50+044513.8 & $>$1.6850 & - & $>$1.24 & 0.34 & 8.46 & 0.70 & 0.032 & 0.425 & 1 & u & 17.38 & - \tabularnewline 
142409.49+043452.1 & 0.6654 & u & $>$1.32 & 0.51 & 7.23 & 0.45 & 0.031 & -0.167 & 1 & u & 13.56 & radio \tabularnewline 
142505.61+035336.2 & 2.2476 & u & $>$1.13 & $<$0.09 & $<$0.57 & - & 0.032 & -0.247 & 1 & u & - & - \tabularnewline 
142526.20$-$011825.8 & - & - & $>$1.05 & 0.41 & $<$4.28 & - & 0.037 & 0.638 & 1 & u & 15.77 & radio \tabularnewline 
143657.71+563924.8 & - & - & 0.99 & 0.41 & 6.06 & 0.95 & 0.063 & -0.166 & 1 & u & 21.6 & radio \tabularnewline 
145111.69+580003.0 & 0.4053 & - & $>$1.13 & 0.39 & $<$3.86 & - & 0.085 & -0.084 & 0.33 & 0.08 & - & - \tabularnewline 
145507.44+025040.3 & - & - & $>$1.01 & 0.62 & 14.42 & 0.80 & 0.035 & 0.351 & 1 & u & 14.01 & radio \tabularnewline 
150006.49+012956.0 & 0.7083 & - & $>$0.92 & 0.34 & $<$2.53 & - & 0.038 & -0.013 & 0.83 & 0.11 & 14.16 & radio \tabularnewline 
150106.26+552750.9 & - & - & $>$1.01 & 0.50 & $<$4.10 & - & 0.052 & 0.069 & 1 & u & - & - \tabularnewline 
150106.26+552750.9 & - & - & $>$1.01 & 0.50 & 5.37 & 0.72 & 0.052 & 0.069 & 1 & u & - & - \tabularnewline 
150818.97+563611.2 & 2.0521 & u & $>$0.95 & $<$0.21 & $<$3.73 & - & 0.083 & 0.229 & 1 & u & - & - \tabularnewline 
151115.49+563715.4 & - & - & $>$1.06 & $<$0.25 & $<$5.05 & - & 0.115 & -0.223 & 1 & u & - & - \tabularnewline 
153058.17+573625.2 & 1.0998 & u & $>$1.08 & 0.50 & 8.07 & 1.11 & 0.085 & -0.437 & 1 & u & 14.93 & - \tabularnewline 
154515.78+003235.2 & 1.0114 & u & $>$1.00 & $<$0.23 & $<$1.79 & - & 0.05 & 0.543 & 1 & u & 24.04 & radio \tabularnewline 
154515.78+003235.2 & 1.0114 & u & $>$1.00 & $<$0.23 & $<$5.56 & - & 0.05 & 0.543 & 1 & u & 24.04 & radio \tabularnewline 
155848.38+022818.6 & - & - & $>$0.96 & 0.48 & 6.56 & 0.57 & 0.034 & -0.28 & 1 & u & - & - \tabularnewline 
160339.49+500955.5 & 0.6209 & u & $>$1.11 & 0.50 & 7.07 & 1.02 & 0.077 & -0.205 & 1 & u & - & - \tabularnewline 
160519.05+542059.9 & 0.2117 & - & 0.81 & 0.36 & 1.68 & 0.70 & 0.056 & 0.297 & 1 & u & 16.19 & radio \tabularnewline 
161541.22+471111.8 & 0.1986 & - & $>$1.35 & 0.52 & 3.55 & 1.16 & 0.081 & 0.225 & 0.53 & 0.05 & - & - \tabularnewline 
162115.21$-$003140.4 & 0.4132 & u & 0.95 & 0.41 & 4.31 & 0.74 & 0.033 & 0.328 & 0.68 & 0.06 & - & - \tabularnewline 
162259.24+440142.9 & - & - & 1.13 & 0.37 & $<$4.93 & - & 0.104 & -0.08 & 1 & u & 17.12 & radio \tabularnewline 
165109.18+421253.5 & 0.2686 & - & $>$1.07 & 0.49 & 3.38 & 1.10 & 0.094 & -0.226 & $<$0.15 & 0.11 & - & - \tabularnewline 
165248.44+363212.6 & 0.6470 & u & $>$1.13 & 0.54 & 8.01 & 0.89 & 0.076 & -0.258 & 1 & u & - & - \tabularnewline 
165806.77+611858.9 & $>$1.4100 & u & $>$1.09 & $<$0.14 & $<$5.52 & - & 0.121 & -0.371 & 1 & u & - & - \tabularnewline 
165806.77+611858.9 & $>$1.4100 & u & $>$1.09 & $<$0.14 & $<$5.59 & - & 0.121 & -0.371 & 1 & u & - & - \tabularnewline 
165808.33+615001.9 & 0.3742 & - & $>$1.19 & 0.47 & 0.86 & 0.27 & 0.042 & 0.027 & 0.64 & 0.10 & - & - \tabularnewline 
170108.90+395443.1 & 1.8900 & u & $>$1.07 & 0.26 & $<$1.20 & - & 0.105 & 0.143 & 1 & u & 23.79 & - \tabularnewline 
170124.64+395437.1 & 0.5071 & u & $>$1.46 & 0.50 & 6.75 & 0.21 & 0.04 & 0.132 & 1 & u & - & - \tabularnewline 
171445.55+303628.0 & 0.8500 & u & 1.14 & 0.25 & $<$0.54 & - & 0.044 & 0.025 & 1 & u & 15.63 & radio \tabularnewline 
171501.36+292912.3 & - & - & $>$0.97 & 0.54 & $<$4.33 & - & 0.116 & -0.069 & 1 & u & - & - \tabularnewline 
172640.50+595550.2 & 0.3471 & u & 1.01 & 0.50 & 2.82 & 1.12 & 0.09 & -0.857 & 1 & u & - & - \tabularnewline 
173719.12+570216.5 & - & - & $>$0.94 & 0.49 & 6.85 & 2.06 & 0.143 & -0.197 & 1 & u & - & - \tabularnewline 
205523.36$-$050619.3 & 0.3426 & - & $>$1.06 & 0.45 & 3.28 & 0.96 & 0.071 & 0.318 & 0.38 & 0.05 & - & - \tabularnewline 
205938.57$-$003756.0 & 0.3354 & - & 0.99 & 0.45 & $<$3.46 & - & 0.071 & 0.257 & 0.37 & 0.06 & - & - \tabularnewline 
211552.88+000115.5 & - & - & $>$0.95 & 0.10 & $<$2.22 & - & 0.073 & 0.102 & 1 & u & - & - \tabularnewline 
211611.89$-$062830.4 & 0.2916 & - & $>$1.08 & 0.41 & 3.56 & 0.85 & 0.071 & -0.086 & 0.37 & 0.11 & - & - \tabularnewline 
212019.13$-$075638.4 & - & - & $>$0.96 & $<$0.23 & $<$3.16 & - & 0.082 & 0.079 & 1 & u & - & - \tabularnewline 
213950.32+104749.6 & 0.2960 & - & 1.02 & - & $<$2.37 & - & 0.073 & 0.646 & 0.11 & 0.04 & - & - \tabularnewline 
215051.73+111916.5 & 0.4946 & u & $>$1.03 & 0.38 & 4.88 & 0.89 & 0.063 & 0.172 & 0.70 & 0.11 & - & - \tabularnewline 
215305.36$-$004230.7 & 0.3416 & - & 0.91 & 0.39 & 5.86 & 0.75 & 0.066 & -0.069 & 0.50 & 0.14 & - & - \tabularnewline 
215650.34$-$085535.4 & $>$1.0179 & u & $>$1.11 & 0.40 & 3.24 & 1.21 & 0.085 & 0.424 & 1 & u & - & - \tabularnewline 
221108.34$-$000302.5 & 0.3619 & - & 0.94 & 0.43 & 6.03 & 0.70 & 0.064 & -0.323 & 0.58 & 0.11 & - & - \tabularnewline 
221109.88$-$002327.5 & 0.4476 & - & $>$0.98 & 0.54 & 5.03 & 0.73 & 0.066 & -0.121 & 0.43 & 0.07 & - & - \tabularnewline 
221456.37+002000.1 & - & - & $>$0.98 & 0.55 & 10.70 & 1.18 & 0.071 & 0.239 & 0.77 & 0.10 & - & - \tabularnewline 
224448.11$-$000619.3 & - & - & $>$0.68 & 0.35 & 4.24 & 0.60 & 0.056 & -0.262 & 1 & u & - & - \tabularnewline 
224730.19+000006.5 & - & - & $>$1.01 & 0.63 & 4.24 & 0.52 & 0.054 & -0.194 & 1 & u & - & - \tabularnewline 
224819.44$-$003641.6 & 0.2123 & - & $>$1.03 & 0.52 & 1.27 & 0.57 & 0.064 & 1.43 & 0.19 & 0.04 & - & - \tabularnewline 
225624.27+130541.7 & - & - & $>$1.10 & 0.49 & 15.56 & 0.80 & 0.058 & -0.038 & 1 & u & - & - \tabularnewline 
231000.81$-$000516.3 & $>$1.6800 & u & $>$1.04 & $<$0.13 & $<$3.21 & - & 0.066 & 0.036 & 1 & u & - & - \tabularnewline 
233445.56+154711.1 & - & - & $>$0.72 & 0.44 & 11.73 & 0.82 & 0.064 & 0.093 & 1 & u & - & - \tabularnewline
235604.03$-$002353.8 & 0.2830 & - & 1.28 & 0.33 & $<$3.48 & - & 0.066 & 0.337 & 0.46 & 0.08 & - & - \tabularnewline
%\end{tabular}
\end{longtable}

